Analyses of Cardinal Auctions

We study cardinal auctions for selling multiple copies of a good, in which bidders specify not only their bid or how much they are ready to pay for the good, but also a cardinality constraint on the number of copies that will be sold via the auction. We perform first known Price of Anarchy type analyses with detailed comparison of the classical Vickrey-Clarke-Groves (VCG) auction and one based on minimum pay property (MPP) which is similar to Generalized Second Price auction commonly used in sponsored search. Without cardinality constraints, MPP has the same efficiency (total value to bidders) and at least as much revenue (total income to the auctioneer) as VCG; this also holds for certain other generalizations of MPP (e.g., prefix constrained auctions, as we show here). In contrast, our main results are that, with cardinality constraints, (a) equilibrium efficiency of MPP is 1/2 of that of VCG and this factor is tight, and (b) in equilibrium MPP may collect as little as 1/2 the revenue of VCG. These aspects arise because in presence of cardinality constraints, more strategies are available to bidders in MPP, including bidding above their value, and this makes analyses nontrivial.

==> 03allocation.tex <==
\section{Finding Optimal Allocation}

For each $k$, define $\Sigma_{k}$ to be maximum value assignment of bidders to at most $k$ positions. Then, we define $k^* = \argmax (\sigma_{k})$. Renumber the advertisers so they are numbered in the decreasing order of their bids. Thus, $b_i$ is the $i$th largest bid, and corresponds now to advertiser renumbered to $i$. 

\begin{lemma}
Define $i_k^*$ to be the smallest $i$ such that $|\{j| j\le i, k_j \ge k\}|=k$, if it exists. Then,
$$ \Sigma_{k} = \sum_{j\le i_k^*, k_j \geq k}  b_j. $$
\end{lemma}

\begin{proof}
The maximum value assignment is simply the maximum bipartite matching of eligible
ads to positions. 
\end{proof}


Our algorithm is simple. We represent each advertiser $i$ by a two dimensional point $(i,p_i)$ with weight $k_i$. Then, we can determine $i_k^*$ by binary searching on $i$ with range query that counts the number of points in $[0,i] \times [k,\infty]$. And we can determine $\Sigma_{k}$ by a single range sum query on $[0,i_k^*] \times [k,\infty]$. Both of these can be answered in $O(\log n)$ time using range searching data structures~\cite{erickson223geometric}. Thus the total running time of the algorithm is $O(n\log n)$ (to sort the bids) + $O(n \log^2 n)$ (for each $k=1,\ldots,n$, we do $O(\log n)$ binary search queries each of which takes $O(\log n)$ time); hence, the total time complexity is $O(n\log^2 n)$. 

\begin{theorem}
There is an $O(n\log^2 n)$ time algorithm to compute $k^*$ and produce an arrangement of ads in $k^*$ slots with
maximum value $\Sigma_{k^{*}}$. 
\end{theorem}

A natural question is if $\Sigma_{k}$ is a single mode function, increasing as $k$ increases from $1$ and decreasing beyond the 
maximum at some $k^*$. If that were the case, the search for $k^*$ would be much more efficient. Unfortunately, that is not true. Consider a sequence of bids $(b_{i},k_{i})$ pairs as follows: 
$$(1000,1),(400,3),(400,3),(400,3), (300,5),(300,5),(300,5),(290,5), (100,5),...$$ 
which produces a see-saw teeth of $\Sigma_{k}$'s: $\Sigma_{1}=1000$, $\Sigma_{1}=800$, $\Sigma_{3}=1200$, $\Sigma_{4}=1190$, etc. We can construct examples with linear number of teeth of maxima if needed.

Another natural question is if $\Sigma_{k^{*}}$ can be computed by simply auctioning one position after another, say going top down, as in~\cite{aggarwal2007bidding}. This is unfortunately incorrect since without fixing a $k$ {\em a priori}, it is impossible to determine the advertisers who compete for any position. 

Thus, we can now compute $b$ to be the max of the two quantities above, plus $\vareps$; we can also easily see that the resulting term will be no larger than $b_i$, and therefore a legal price. This gives, 

\begin{theorem}
MPP price for any advertiser $i$ can be computed in $O(\log n)$ time. Over all advertisers, price computations take $O(n\log n)$ time. 
\end{theorem}

For comparison, one might wish to consider Vickrey-Clarke-Groves (VCG) pricing~\cite{V,C,G}.  Consider any $i$ in $\sigma_{k^{*}}^{*}$. It's VCG price can be seen to be 
$$\Sigma_{k^{*}}^{*}-b_i-\max\{ \max_{\ell < \alpha_i} \Sigma_{\ell}^{*}, \max_{\alpha_i \leq \ell \leq \beta_i} \Sigma_{\ell,+1}^{*}, 
\max_{\beta_i < \ell} \Sigma_{\ell}^{*} \},$$
 which can again be computed in $O(\log n)$ time. 

\medskip
\noindent
{\bf Remark.}
Say there is an upper bound $\ell$ on the number of slots that the bidders are
allowed to specify, as determined by the auctioneer (the search company). Then our 
auction can be implemented in $O(n\ell)$ time easily by considering each potential $k$ of total slots from $1$ to $\ell$. However the implementation we have described above 
is more efficient for large $\ell$ (note that in theory, $\ell$ may be as high as $n$). 

